Entropy and Its Variational Principle for Locally Compact Metrizable Systems

For a given topological dynamical system $(X,T)$ over a compact set $X$ with a metric $d$, the "variational principle" states that \begin{equation*} \sup_{\mu}h_\mu(T) = h(T) = h_d(T), \end{equation*} where $h_\mu(T)$ is the Kolmogorov-Sinai entropy, with the supremum taken over every $T$-invariant probability measure, $h_d(T)$ is the Bowen entropy, and $h(T)$ is the topological entropy as defined by Adler, Konheim and McAndrew. In [9], the concept of topological entropy was adapted for the case where $T$ is a proper map and $X$ is locally compact separable and metrizable, and the variational principle was extended to \begin{equation*} \sup_{\mu}h_\mu(T) = h(T) = \min_d h_d(T), \end{equation*} where the minimum is taken over every distance compatible with the topology of $X$. In the present work, we dropped the properness assumption, extending the above result for any continuous map $T$. We also apply our results to extend some previous formulas for the topological entropy of continuous endomorphisms of connected Lie groups proved in [4]. In particular, we prove that any linear transformation $T: V \to V$ over a finite dimensional vector space $V$ has null topological entropy.

==> definitions.tex <==
\RequirePackage{mathrsfs} % Font \mathscr

\theoremstyle{plain}


\newtheorem{theorem}{Theorem}[section]

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{affirmation}{Claim}
\newenvironment{proofitemenv}
  {\par\noindent\vspace{10pt}\rule{1ex}{1ex}\hspace{2ex}} %TODO: clear left.
  {\par}
\newtheorem{case}{Case}
\newtheorem*{notation}{Notation}
\newtheorem{definition}[theorem]{Definition}

% Horrível: o estilo "definition" não é bom para definição e notação!
% Horrível: estilo "remark" é ruim para observações e exemplos!!
\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{obs}[theorem]{Remark}
%\newtheorem{problem}{Problema}

%% Quadradinho no final das demonstrações.
%\renewcommand{\qedsymbol}{$\blacksquare$}

\providecommand{\email}[1]{{#1}}


%Divides de proof into cases. (TODO: not good yet.)
\newlength{\affrule}
\providecommand{\subproof}[2]
{{
  \begin{quote}
    \begin{affirmation}
      {#1}
    \end{affirmation}

    \parindent .5cm %\parskip .2cm
    {#2}
  \end{quote}
  \vspace{10pt}
}}

\providecommand{\subcase}[2]
{{
  \vspace{10pt}
  \begin{case}
    {#1}
  \end{case}

  {#2}
}}

\providecommand{\proofitem}[2]
{{
  \vspace{15pt}
  \begin{proofitemenv}
    {#1}
  \end{proofitemenv}

  {#2}
}}


%Não sei se é o latex ou se sou eu, mas as "referências" não têm a cara certa!
\providecommand{\refeq}[1]{{(\ref{#1})}}
\providecommand{\refitem}[1]{{(\ref{#1})}}

%comment
\providecommand{\comentario}[2][APAGADO!!]{{#1}}


%% TODO: Trocar por \R \N \Z \T, etc. (como em 2/definitions_01.tex)
% Commonly used sets.
\providecommand{\naturals}[0]{\mathbb{N}}
\providecommand{\integers}[0]{\mathbb{Z}}
\providecommand{\rationals}[0]{\mathbb{Q}}
\providecommand{\reals}[0]{\mathbb{R}}
\providecommand{\nonnegativereals}[0]{\mathbb{R^+}}
\providecommand{\complexes}[0]{\mathbb{C}}
\providecommand{\torus}[0]{\mathbb{T}}
\providecommand{\projective}[0]{\mathbb{P}}
\providecommand{\timeset}[0]{\mathbb{T}}

\providecommand{\family}[1]{{\mathscr{#1}}}
\providecommand{\parts}[1]{{\family{P}\left(#1\right)}}
\providecommand{\neighbourhoods}[1]{{\family{V}\left(#1\right)}}
\providecommand{\generatedtopology}[1]{{\tau\left(#1\right)}}
\providecommand{\generatedtopologybase}[1]{{\family{B}\left(#1\right)}}

%\providecommand{\liealgebra}[1]{\textgoth{#1}}
%\providecommand{\liealgebra}[1]{\textfrak{#1}}
\providecommand{\liealgebra}[1]{\mathfrak{#1}}
%\providecommand{\liealgebra}[1]{\textswab{#1}}


% Special symbols.
\providecommand{\suchthat}[0]{{\thickspace | \thickspace}}
\providecommand{\cardinality}[1]{{\# #1}}

% Brackets.
\newcommand{\threebracket}[5]{{\left #1 \vphantom{{#2}^N}\vphantom{{#4}^N}{#2} \, \right #3 \left. \vphantom{{#2}^N}\vphantom{{#4}^N}{#4} \right #5}}

\providecommand{\setsuchthat}[2]{{\threebracket{\{}{#1}{|\:}{#2}{\}}}}
\providecommand{\set}[1]{{\left \{ {#1} \right \}}}
\providecommand{\abs}[1]{{\left\lvert#1\right\rvert}}
\providecommand{\norm}[2][]{{\left\lVert{#2}\right\rVert_{#1}}}

\newcommand{\integral}[3][]{{\int_{#1} {#2}\, \mathrm{d}{#3}}}
\newcommand{\conditionalexpectation}[2]{{E \threebracket{(}{#1}{|}{#2}{)}}}
\newcommand{\qtp}[1]{{[{#1}-\qtpop]}}

% Operator names.
\DeclareMathOperator{\identity}{id}
\DeclareMathOperator{\interiorop}{int}
\DeclareMathOperator{\closureop}{cl}
\DeclareMathOperator{\supportop}{supp}
\DeclareMathOperator{\qtpop}{qtp}

\DeclareMathOperator{\eigenspace}{eig}
\DeclareMathOperator{\expbase}{e}


% Functions
\newcommand{\function}[3]{{#1: #2 \to #3}}
\newcommand{\functionmaps}[3]{{#1: #2 \mapsto #3}}
\newcommand{\functionarray}[5]{{\begin{array}[t]{lrcl}
                                  #1:& #2 &\to     &#3 \\
                                     & #4 &\mapsto &#5
                                \end{array}}}

% Operations
\newcommand{\closure}[1]{{\overline{#1}}}
%\newcommand{\closure}[1]{{\closureop \left({#1}\right)}}
%\newcommand{\interior}[1]{{\mathring{#1}}}
\newcommand{\interior}[1]{\interiorop \left({#1}\right)}
\newcommand{\complementset}[1]{{#1}^{c}}
\newcommand{\powerset}[1]{{\mathscr{P}({#1})}}
\newcommand{\indicator}[1]{{I_{#1}}}
\newcommand{\support}[1]{{\supportop \left( {#1} \right)}}

\newcommand{\transposedmatrix}[1]{{#1}^{T}}


\newcommand{\ball}[3][]{{B_{#1}\left({#3}; {#2}\right)}}
\newcommand{\balls}[2]{{\family{B}_{#1}\left({#2}\right)}}

\newcommand{\diagonal}[1][]{{\Delta_{#1}}}


% Eca!!!
\DeclareMathOperator{\Gl}{Gl}
\newcommand{\gl}{{\mathfrak{gl}}}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\newcommand{\recurrent}{{\mathcal{R}}}
\newcommand{\chainrecurrent}{{\mathcal{R}_c}}
\DeclareMathOperator{\fix}{fix}


% Matrix
% TODO: Substituir primeiro argumento por número.
\newcommand{\Matrix}[2]{\left( \begin{array}{#1}#2\end{array} \right)}


\newcommand{\covercardinality}[2][]{{N_{#1}\left({#2}\right)}}
\newcommand{\separatedcardinality}[3]{{s\left({#1}, {#2}, {#3}\right)}}

\newcommand{\radonprobabilities}[1]{{\mathcal{P}\left({#1}\right)}}
\newcommand{\invariantradonprobabilities}[2]{{\mathcal{P}_{{#1}}\left({#2}\right)}}
\newcommand{\radonmeasures}[1]{{\mathcal{M}\left({#1}\right)}}
\newcommand{\invariantradonmeasures}[2]{{\mathcal{M}_{{#1}}\left({#2}\right)}}
\newcommand{\radonball}[1]{{\mathcal{B}\left({#1}\right)}}
\newcommand{\invariantradonball}[2]{{\mathcal{B}_{{#1}}\left({#2}\right)}}

\newcommand{\dynamicalsystem}[2]{{\function{#2}{#1}{#1}}}

\newcommand{\borelsets}[0]{{\family{B}}}
\newcommand{\measurablesets}[1]{{\family{B}}}
\newcommand{\measurablespace}[1]{{\left({#1}, \measurablesets{#1}\right)}}
\newcommand{\probability}[1]{{\mu}}
\newcommand{\measure}[1]{{\mu}}
\newcommand{\probabilityspace}[1]{{\left({#1}, \measurablesets{#1}, \probability{#1}\right)}}
\newcommand{\measurespace}[1]{{\left({#1}, \measurablesets{#1}, \measure{#1}\right)}}


\newcommand{\partitionentropy}[2]{{H_{#1}\left({#2}\right)}}
\newcommand{\tpartitionentropy}[3]{{h_{#1}\left({#3}, {#2}\right)}}
\newcommand{\measureentropy}[2]{{h_{#1}\left({#2}\right)}}

\newcommand{\conditionalprobability}[3]{{{#1}\threebracket{(}{#3}{|}{#2}{)}}}
\newcommand{\conditionalpartitionentropy}[3]{{H_{#1}\threebracket{(}{#2}{|}{#3}{)}}}

%\newcommand{\topology}[1]{{\tau}}
%\newcommand{\topologicalspace}[1]{{\left({#1}, \topology{#1}\right)}}
\newcommand{\topologicalspace}[1]{{#1}}

\newcommand{\metricspace}[2]{{\left({#1}, {#2}\right)}}
\newcommand{\iteratedmetric}[2]{{{#1}_{#2}}}

\newcommand{\coverentropy}[1]{{H\left({#1}\right)}}
\newcommand{\tcoverentropy}[2]{{h\left({#2}, {#1}\right)}}

\newcommand{\topologicalentropy}[1]{{h\left({#1}\right)}}

%\newcommand{\ksentropy}[1]{{h_{ks}\left({#1}\right)}}
\newcommand{\ksentropy}[2][\mu]{{\sup_{#1} \measureentropy{#1}{{#2}}}}

\newcommand{\bowenentropy}[2]{{h_{#1}\left({#2}\right)}}
\newcommand{\dentropy}[2]{{h^{#1}\left({#2}\right)}}
\newcommand{\epsilonbowenentropy}[4]{{h_{#1}\left({#2}, {#3}, {#4}\right)}}
\newcommand{\epsilondentropy}[3]{{h^{#1}\left({#2}, {#3}\right)}}


\newcommand{\pinsker}[1][]{{\family{P}_{#1}}}

\newcommand{\continuousfunctions}[1]{{C\left(#1\right)}}
\newcommand{\compactsuportfunctions}[1]{{C_c\left(#1\right)}}
\newcommand{\vanishingatinfinityfunctions}[1]{{C_0\left(#1\right)}}


\newcommand{\compactification}[1]{{\widetilde{#1}}}
\newcommand{\onepointcompactification}[1]{{{#1}^*}}

